Challenges and Opportunities for the Design of Smart Speakers

Advances in voice technology and voice user interfaces (VUIs) -- such as Alexa, Siri, and Google Home -- have opened up the potential for many new types of interaction. However, despite the potential of these devices reflected by the growing market and body of VUI research, there is a lingering sense that the technology is still underused. In this paper, we conducted a systematic literature review of 35 papers to identify and synthesize 127 VUI design guidelines into five themes. Additionally, we conducted semi-structured interviews with 15 smart speaker users to understand their use and non-use of the technology. From the interviews, we distill four design challenges that contribute the most to non-use. Based on their (non-)use, we identify four opportunity spaces for designers to explore such as focusing on information support while multitasking (cooking, driving, childcare, etc), incorporating users' mental models for smart speakers, and integrating calm design principles.

==> random.tex <==
\makeatletter
\let\oldlt\longtable
\let\endoldlt\endlongtable
\def\longtable{\@ifnextchar[\longtable@i \longtable@ii}
\def\longtable@i[#1]{\begin{figure}[t]
\onecolumn
\begin{minipage}{0.5\textwidth}
\oldlt[#1]
}


\def\longtable@ii{\begin{figure}[t]
\onecolumn
\begin{minipage}{0.5\textwidth}
\oldlt
}


\def\endlongtable{\endoldlt
\end{minipage}
\twocolumn
\end{figure}}
\makeatother

==> table_lit_arxivsave.tex <==
% Please add the following required packages to your document 
% \begin{tabular}{|p{1cm}|p{1cm}|p{5in}|}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:

% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly\begin{table}[]
{\renewcommand{\arraystretch}{1.25}

% \begin{table*}

\begin{table*}
\captionsetup{justification=centering}
\space\space \caption{Lit Review Themes and Example Guidelines
\\ \textit{Note: The number (\#) inside the parentheses indicates how many guidelines belong to the theme.}}
{\small
\begin{longtable}{|P{1.6cm}|P{2.7cm}|p{12.5cm}|}

% \small\begin{longtable}{|m{1.3cm}|m{2.2cm}|p{10.75cm}|}
% \begin{longtable}{|c|c|l|}
\hline
  \textbf{Themes} &
  \textbf{Sub-themes} &
  \textbf{Example Guidelines} \\ \hline
\endfirsthead
%
\endhead
\multirow{12}{*}{
% \setlength\extrarowheight{-10pt
% Spread rows out...
\begin{tabular}[c]{@{}c@{}}\\\\\\\\\\\\\textbf{Enhance} \\\textbf{Basic}\\ \textbf{Usability}\\ \textbf{(51)}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\Promote\\Error Prevention (20)\end{tabular}} &
 
 A12. Confirm input intelligently: [current VUIs] failed to explicitly confirm some critical actions [, like double-checking which alarm to turn off]  \cite{wei_evaluating_2018}.\\ \cline{3-3} 
 &
   &
   
 [VUIs] need to provide feedback to the user explaining their interpretation of the [ambiguous or underspecified utterance] and how it was handled \cite{setlur_how_2022}.  \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Strengthen\\ User Control (13)\end{tabular}} &
  Provide ability for users to control and interrupt \cite{vacher_evaluation_2015}. \\ \cline{3-3} 
 &
   &
  The control users have on the processing of their actions by the system. \cite{nowacki_improving_2020}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.25cm]Leverage \\Multimodality (7)\end{tabular}} &
  Address {[}low situation awareness{]} by providing better vocal feedback... and adding visual indication for information that is critical to the user \cite{luria} \\ \cline{3-3} 
 &
   &
  Leverage task context and multimodality in order to provide visual or other non-verbal cues \cite{axtell_tea_2021}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.25cm]Improve\\ Compatibility (4)\end{tabular}} &
  Smart Home Framework: the compatibility of the [VUIs] with smart home devices \cite{lopez_alexa_2018}. \\ \cline{3-3} 
 &
   &
  Integrate {[}the VUIs with{]} not only smartphones but also connected televisions, computers, and other screen-based devices \cite{sciutojasonhong}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\Enhance\\ Discoverability (4)\end{tabular}} &
  Use responses to help users discover what is possible...rather than always say something is impossible: the system did not teach ways to ask for a result, and {[}users{]} had to guess and try multiple times \cite{wei_evaluating_2018}. \\ \cline{3-3} 
 &
   &
  Data mining to offer new features: ...significant challenge for [VUIs]. One opportunity is to data mine repeated patterns of use or use common routines as scaffolding to introduce new related features \cite{sciutojasonhong}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.25cm]Facilitate\\ Error Recovery (3)\end{tabular}} &
  Provide interface affordances (visual or language) so users can refine and repair system choices \cite{setlur_how_2022}. \\ \cline{3-3} 
 &
   &
  A17. Allow users to exit from errors or a mistaken conversation: Use a special escape word globally (e.g. "Stop")... {[}or{]} non-speech methods when speech fails (e.g., push a physical button) \cite{wei_evaluating_2018}. \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\\\\\\\\\textbf{Customize}\\ \textbf{for User}\\ \textbf{Context}\\ \textbf{(26)}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ Remember\\Usage History (13)\end{tabular}} &
  Remember User Profiles to Deliver Personalized Services: store a vast amount of information specific to the user, such as personal profiles or preferences \cite{kim_designers_2021} \\ \cline{3-3} 
 &
   &
  Enable user to employ territorial markers to help them avoid activity- and preference-related conflicts by communicating their preferences or staking a claim to the device or data \cite{gargindian}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Design for\\ Diverse \& Sensitive\\ Populations (9)\end{tabular}} &
  Enriching the responding contents when executing these commands might give older adults a chance to find more features and functionalities \cite{kim_exploring_2021}.
  \\ \cline{3-3} 
 &
   &
  Adopt social-justice oriented design methods...when building [VUIs] in home health care contexts \cite{bartle_second_2022}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.25cm]Leverage\\ User's\\ Environment (4)\end{tabular}} &
 {Integrate the functionality of ubicomp sensors: install additional sensors in the home that can serve as automatic warning alarms, for example, if the stove is left on or if there is a water leak. {[}or{]} whether someone is within earshot before triggering interactions \cite{reddy_making_2021}}.  \\ \cline{3-3} 
 &
   &
  Leverage knowledge of place: {[}As the VUIs{]} is in a living room versus a bedroom, it can modify its level of proactivity, listen for particular commands, and offer suggestions for new uses \cite{nowacki_improving_2020}. \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\\\\[-0.25cm]\textbf{Speak}\\\textbf{Users'}\\\textbf{Language}\\ \textbf{(24)}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.25cm] Accommodate\\ Conversational\\ Speech (18)\end{tabular}} &
  Enhancing the message interactivity of the human-{[}VUIs{]} conversation by increasing the degree of contingency in message exchanges \cite{wang_alexa_2020}. \\ \cline{3-3} 
 &
   &
  Tailor responses and follow-up questions to make interactions more engaging, elicit in-depth disclosure, and effectively provide emotional support through these devices most natural responses \cite{shani_alexa_2022}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.25cm] Anthropomorphize\\ Human's Emotions (6)\end{tabular}} &
  Employ empathetic expressions to show emotional responsiveness. When [VUIs] use phrases such as "I understand" or "I can relate to you"... users are likely to perceive it being highly social \cite{wang_alexa_2020}. \\ \cline{3-3} 
 &
   &
  Express Sympathy; Be Interesting, Charming, and Lovable; Express Interest to Users \cite{sabir_hey_2022}. \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.25cm]\textbf{Design for}\\\textbf{Simpler}\\ \textbf{Interactions}\\ \textbf{(16)}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.25cm]Design for Shorter\\ Conversation (8)\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Design for short interactions, know when it will be long: Systems can prepare for the large majority\\ of interactions to be a single command-answer or command-action \cite{axtell_tea_2021}.\end{tabular} \\ \cline{3-3} 
 &
   &
  A11. Keep feedback and prompts short: ... the {[}current VUIs'{]} responses were not always clear or succinct, making it difficult for users to listen, understand, and remember \cite{wei_evaluating_2018}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Design for Simpler\\ Conversation (8)\end{tabular}} &
Guide users through a conversation so they are not easily lost \cite{murad_revolution_2019}.\\ \cline{3-3} 
 &
   &
    Minimize acoustic confusability of vocabulary \cite{wei_evaluating_2018}.\\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\\textbf{Establish}\\\textbf{Trust}\\ \textbf{(10)}\end{tabular}} &
  \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}
 \\\\[-0.25cm] Establish\\Trust (10)\end{tabular}} &
 Where available, tangible controls can improve the privacy experience \cite{kim_designers_2021}. \\ \cline{3-3} 
 & &
  Acknowledgments and confirmations: To build trust, acknowledgments need to be provided as feedback indicating that the user’s input was received \cite{alrumayh_context_2020}. \\ \cline{3-3} 
  & &
  Explicitly including a warning message about a third-party vendor in Alexa’s initial response to activating a third-party skill \cite{zubatiy_empowering_2021}. \\ 
 
  
  \hline
\end{longtable}}
\end{table*}

}

==> table_lit_old.tex <==
% Please add the following required packages to your document 
% \begin{tabular}{|p{1cm}|p{1cm}|p{5in}|}

\clearpage
\onecolumn

% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:

% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly\begin{table}[]
\renewcommand{\arraystretch}{1.05}
{\footnotesize
\begin{longtable}{|P{1.4cm}|P{2.4cm}|p{10.05cm}|}
\captionsetup{justification=centering}
\space\space \caption{Lit Review Themes and Example Guidelines
\\ \textit{Note: The number (\#) inside the parentheses indicates how many guidelines belong to the theme.}}
% \small\begin{longtable}{|m{1.3cm}|m{2.2cm}|p{10.75cm}|}
% \begin{longtable}{|c|c|l|}
\hline
  \textbf{Themes} &
  \textbf{Sub-themes} &
  \textbf{Example Guidelines} \\ \hline
\endfirsthead
%
\endhead
%
\multirow{12}{*}{
% \setlength\extrarowheight{-10pt
% Spread rows out...
\begin{tabular}[c]{@{}c@{}}\\\\\\\\\\\\\\\\\\\\\textbf{Enhance} \\\textbf{Basic}\\ \textbf{Usability}\\ \textcolor{blue}{\textbf{(61)}}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\Promote\\Error Prevention (21)\end{tabular}} &
 
 A12. Confirm input intelligently: [current VUIs] failed to explicitly confirm some critical actions [, like double-checking which alarm to turn off]  \cite{wei_evaluating_2018}.\\ \cline{3-3} 
 &
   &
   
 [VUIs] need to provide feedback to the user explaining their interpretation of the [ambiguous or underspecified utterance] and how it was handled \cite{setlur_how_2022}.  \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Strengthen\\ User Control (13)\end{tabular}} &
  Provide ability for users to control and interrupt \cite{vacher_evaluation_2015}. \\ \cline{3-3} 
 &
   &
  The control users have on the processing of their actions by the system. \cite{nowacki_improving_2020}. \\ \cline{2-3}
  &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textcolor{blue}{\\ \\\textcolor{blue}{Provide}\\ \textcolor{blue}{Feedback (9)}}\end{tabular}} &
   \textcolor{blue}{Add additional feedback currently the {[}VUIs{]} says “I will remind you” if you set a reminder, but perhaps it could also have an external visual cue that is active only if there is still a pending reminder. This additional feedback would minimize the need for participants to repeatedly ask what their reminders are and could contribute to building trust with the {[}VUI{]} system \cite{reddy_making_2021}.} \\ \cline{3-3} 
 &
   &
 \textcolor{blue}{Acknowledgments and confirmations: To build trust, acknowledgments need to be provided as feedback indicating that the user’s input was received \cite{alrumayh_context_2020}.} \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.2cm]Leverage \\Multimodality (7)\end{tabular}} &
  Address {[}low situation awareness{]} by providing better vocal feedback... and adding visual indication for information that is critical to the user \cite{luria} \\ \cline{3-3} 
 &
   &
  Leverage task context and multimodality in order to provide visual or other non-verbal cues \cite{axtell_tea_2021}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.2cm]Improve\\ Compatibility (4)\end{tabular}} &
  Smart Home Framework: the compatibility of the [VUIs] with smart home devices \cite{lopez_alexa_2018}. \\ \cline{3-3} 
 &
   &
  Integrate {[}the VUIs with{]} not only smartphones but also connected televisions, computers, and other screen-based devices \cite{sciutojasonhong}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\Enhance\\ Discoverability (4)\end{tabular}} &
  Use responses to help users discover what is possible...rather than always say something is impossible: the system did not teach ways to ask for a result, and {[}users{]} had to guess and try multiple times \cite{wei_evaluating_2018}. \\ \cline{3-3} 
 &
   &
  Data mining to offer new features: ...significant challenge for [VUIs]. One opportunity is to data mine repeated patterns of use or use common routines as scaffolding to introduce new related features \cite{sciutojasonhong}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.2cm]Facilitate\\ Error Recovery (3)\end{tabular}} &
  Provide interface affordances (visual or language) so users can refine and repair system choices \cite{setlur_how_2022}. \\ \cline{3-3} 
 &
   &
  A17. Allow users to exit from errors or a mistaken conversation: Use a special escape word globally (e.g. "Stop")... {[}or{]} non-speech methods when speech fails (e.g., push a physical button) \cite{wei_evaluating_2018}. \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\\\\\\\\\textbf{Customize}\\ \textbf{for User}\\ \textbf{Contexts}\\ \textbf{(23)}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\ Remember\\Usage History (13)\end{tabular}} &
  Remember User Profiles to Deliver Personalized Services: store a vast amount of information specific to the user, such as personal profiles or preferences \cite{kim_designers_2021} \\ \cline{3-3} 
 &
   &
  Enable user to employ territorial markers to help them avoid activity- and preference-related conflicts by communicating their preferences or staking a claim to the device or data \cite{gargindian}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Design for\\ Diverse \& Sensitive\\ Populations (6)\end{tabular}} &
  Enriching the responding contents when executing these commands might give older adults a chance to find more features and functionalities \cite{kim_exploring_2021}.
  \\ \cline{3-3} 
 &
   &
  Adopt social-justice oriented design methods...when building [VUIs] in home health care contexts \cite{bartle_second_2022}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\Leverage\\ User's\\ Environment (4)\end{tabular}} &
 {Integrate the functionality of ubicomp sensors: install additional sensors in the home that can serve as automatic warning alarms, for example, if the stove is left on or if there is a water leak. {[}or{]} whether someone is within earshot before triggering interactions \cite{reddy_making_2021}}.  \\ \cline{3-3} 
 &
   &
  Leverage knowledge of place: {[}As the VUIs{]} is in a living room versus a bedroom, it can modify its level of proactivity, listen for particular commands, and offer suggestions for new uses \cite{nowacki_improving_2020}. \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\\\\[-0.2cm]\textbf{Speak}\\\textbf{Users'}\\\textbf{Language}\\ \textbf{(23)}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.2cm]Accommodate\\ Conversational\\ Speech (17)\end{tabular}} &
  Enhancing the message interactivity of the human-{[}VUIs{]} conversation by increasing the degree of contingency in message exchanges \cite{wang_alexa_2020}. \\ \cline{3-3} 
 &
   &
  Tailor responses and follow-up questions to make interactions more engaging, elicit in-depth disclosure, and effectively provide emotional support through these devices most natural responses \cite{shani_alexa_2022}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.2cm]Anthropomorphize\\ Human's Emotions (6)\end{tabular}} &
  Employ empathetic expressions to show emotional responsiveness. When [VUIs] use phrases such as "I understand" or "I can relate to you"... users are likely to perceive it being highly social \cite{wang_alexa_2020}. \\ \cline{3-3} 
 &
   &
  Express Sympathy; Be Interesting, Charming, and Lovable; Express Interest to Users \cite{sabir_hey_2022}. \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.2cm]\textbf{Design for}\\\textbf{Simpler}\\ \textbf{Interactions}\\ \textbf{(16)}\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\\[-0.2cm]Design for Shorter\\ Conversation (8)\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}Design for short interactions, know when it will be long: Systems can prepare for the large majority\\ of interactions to be a single command-answer or command-action \cite{axtell_tea_2021}.\end{tabular} \\ \cline{3-3} 
 &
   &
  A11. Keep feedback and prompts short: ... the {[}current VUIs'{]} responses were not always clear or succinct, making it difficult for users to listen, understand, and remember \cite{wei_evaluating_2018}. \\ \cline{2-3} 
 &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Design for Simpler\\ Conversation (8)\end{tabular}} &
  Minimize acoustic confusability of vocabulary \cite{wei_evaluating_2018}.\\ \cline{3-3} 
 &
   &
  Guide users through a conversation so they are not easily lost \cite{murad_revolution_2019} \\
\hline
\end{longtable}
}

==> table_result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly

\renewcommand{\arraystretch}{1.05}
% \small{
\begin{longtable}{|P{0.1cm}|P{5.2cm}|P{5.2cm}|p{3.05cm}|}
\space\space \caption{\textcolor{blue}{Opportunities and Challenges Matrix with Literature Review Insights}}
\hline
 &
  Opportunities &
  Challenges &
  Literature Review \\ \hline
\endfirsthead
%
\endhead
%
% \multirow{2}{*}{1} &
%   \multirow{2}{*}{
%   Explore Use Cases to Understand and Support\textit{Information} While \textit{Primary Task}} &
%   Unmatched Expectation for Task Complexity &
%   \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Customize for User Context\\ Design for Diverse Population\end{tabular}} \\ \cline{3-3}
% &
%   &
%  Unmatched Expectation for Input Efficiency &
%   \\ \hline
1 &
  Explore Use Cases to Understand and Support \textit{Information} While \textit{Primary Task} &
  \begin{tabular}[c]{@{}c@{}}Unmatched Expectation for Task Complexity\\ Unmatched Expectation for Input Efficiency\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Customize for User Context\\ Design for Diverse Population\end{tabular} \\ \hline
2 &
  Focus on Short Commands rather than Extended Conversations &
  Unmatched Expectation for Task Complexity &
  Design for Simpler Interactions \\ \hline
3 &
  Improve Input Efficiency by Learning User Preferences &
  Unmatched Expectation for Input Efficiency &
  Customize for User Context \\ \hline
4 &
  Improve Discoverability by Promoting Social Learning from Observations and Tutorial Videos &
  Poor Discoverability &
  Discoverability \\ \hline
5 &
    / & 
  Trust \& Privacy &
  Establish Trust \\ \hline
6 &
    / &
  Lack of Affective Responsiveness &
  Speak Users' Language \\ \hline

\end{longtable}

